HEX: Hierarchical Emergence Exploitation in Self-Supervised Algorithms

In this paper, we propose an algorithm that can be used on top of a wide variety of self-supervised (SSL) approaches to take advantage of hierarchical structures that emerge during training. SSL approaches typically work through some invariance term to ensure consistency between similar samples and a regularization term to prevent global dimensional collapse. Dimensional collapse refers to data representations spanning a lower-dimensional subspace. Recent work has demonstrated that the representation space of these algorithms gradually reflects a semantic hierarchical structure as training progresses. Data samples of the same hierarchical grouping tend to exhibit greater dimensional collapse locally compared to the dataset as a whole due to sharing features in common with each other. Ideally, SSL algorithms would take advantage of this hierarchical emergence to have an additional regularization term to account for this local dimensional collapse effect. However, the construction of existing SSL algorithms does not account for this property. To address this, we propose an adaptive algorithm that performs a weighted decomposition of the denominator of the InfoNCE loss into two terms: local hierarchical and global collapse regularization respectively. This decomposition is based on an adaptive threshold that gradually lowers to reflect the emerging hierarchical structure of the representation space throughout training. It is based on an analysis of the cosine similarity distribution of samples in a batch. We demonstrate that this hierarchical emergence exploitation (HEX) approach can be integrated across a wide variety of SSL algorithms. Empirically, we show performance improvements of up to 5.6% relative improvement over baseline SSL approaches on classification accuracy on Imagenet with 100 epochs of training.

==> Tables/dataset_comparison.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccc}
                & \multicolumn{2}{c}{SimCLR} & \multicolumn{2}{c}{SimCLR + HEX} \\ \cline{2-5} 
Dataset         & Top-1        & Top-5       & Top-1           & Top-5          \\ \hline

iNat21     \cite{van2018inaturalist}     &     20.67         &     38.64        &        \textbf{22.01}         &       \textbf{40.92}         \\
TinyImageNet-200 \cite{yao2015tiny} &      40.92        &    68.02         &       \textbf{45.35}          &       \textbf{70.89}         \\
STL-10     \cite{coates2011analysis}      &       86.16       &       99.34      &        \textbf{88.83}         &     \textbf{99.51}              \\
Cifar-10   \cite{krizhevsky2009learning}       &    89.17          &  99.72         &   \textbf{90.59}              &        \textbf{99.73}        \\\hline
\end{tabular}}
\caption{Performance of HEX on top of SimCLR across a wide variety of datasets of varying complexity in a linear evaluation setting. The stepwise thresholding strategy is used for HEX in this table.}
\label{tab: dataset}
\end{table}

==> Tables/imagenet_comparison.tex <==
\begin{table}[]
\centering
\begin{tabular}{clcc}
                                 &      & \multicolumn{2}{c}{ImageNet}                \\ \cline{3-4} 
Method                           & Type & Top-1                  & Top-5                \\ \hline
SimCLR                           &  N/A    &  57.74                    &            81.44          \\
\multicolumn{1}{l}{SimCLR + HEX} &  Adaptive    & 
\multicolumn{1}{l}{\textbf{59.03}} & \multicolumn{1}{l}{\textbf{82.83}} \\ 

\hline

NNCLR                           &    N/A  &  62.47                    &         85.13             \\
\multicolumn{1}{l}{NNCLR + HEX} &  Adaptive    & 
\multicolumn{1}{l}{\textbf{65.96}} & \multicolumn{1}{l}{\textbf{87.02}} \\ 

\hline
\end{tabular}
\caption{Performance of HEX on the ImageNet dataset within a linear evaluation setting.}
\label{tab: imagenet}
\end{table}

==> Tables/semi_supervised.tex <==
\begin{table}[]
\centering
\begin{tabular}{clcc}
                                 &      & \multicolumn{2}{c}{ImageNet}                \\ \cline{3-4} 
Method                           & Type & 1\%                  & 10\%                \\ \hline
SimCLR                           &  N/A    &  29.61                    &       47.85               \\
\multicolumn{1}{l}{SimCLR + HEX} &  Adaptive    & 
\multicolumn{1}{l}{\textbf{33.72}} & \multicolumn{1}{l}{\textbf{50.48}} \\ 

\hline

NNCLR                           &    N/A  &       39.94             &             57.83         \\
\multicolumn{1}{l}{NNCLR + HEX} &  Adaptive    & 
\multicolumn{1}{l}{\textbf{46.00}} & \multicolumn{1}{l}{\textbf{61.45}} \\ 

\hline
\end{tabular}
\caption{This table shows a semi-supervised fine-tuning evaluation of HEX models with access to 1\% and 10\% subsets of the ImageNet during fine-tuning. The metric is top-1 accuracy.}
\label{tab: semi}
\end{table}

==> Tables/superclass.tex <==
\begin{table}[]
\centering
\begin{tabular}{ccc}
\hline
Method       & \begin{tabular}[c]{@{}c@{}}Decomposition\\ Type\end{tabular} & Cifar-100 Test Set \\ \hline
SimCLR       & N/A                                                          & 64.46              \\
SimCLR + HEX & SuperClass                                                   & \textbf{69.01}              \\ \hline
NNCLR        & N/A                                                          & 70.72              \\
NNCLR + HEX  & SuperClass                                                   & \textbf{74.04}              \\ \hline
All4One      & N/A                                                          & 72.48              \\
All4One + HEX     & SuperClass                                                   & \textbf{73.82}              \\ \hline
\end{tabular}
\caption{Performance of our method in a linear evaluations setting under the assumption that the 20 superclass labels are fully available on the Cifar-100 dataset.}
\label{tab: superclass}
\end{table}
